SynthWorlds: Controlled Parallel Worlds for Disentangling Reasoning and Knowledge in Language Models

Evaluating the reasoning ability of language models (LMs) is complicated by their extensive parametric world knowledge, where benchmark performance often reflects factual recall rather than genuine reasoning. Existing datasets and approaches (e.g., temporal filtering, paraphrasing, adversarial substitution) cannot cleanly separate the two. We present SynthWorlds, a framework that disentangles task reasoning complexity from factual knowledge. In SynthWorlds, we construct parallel corpora representing two worlds with identical interconnected structure: a real-mapped world, where models may exploit parametric knowledge, and a synthetic-mapped world, where such knowledge is meaningless. On top of these corpora, we design two mirrored tasks as case studies: multi-hop question answering and page navigation, which maintain equal reasoning difficulty across worlds. Experiments in parametric-only (e.g., closed-book QA) and knowledge-augmented (e.g., retrieval-augmented) LM settings reveal a persistent knowledge advantage gap, defined as the performance boost models gain from memorized parametric world knowledge. Knowledge acquisition and integration mechanisms reduce but do not eliminate this gap, highlighting opportunities for system improvements. Fully automatic and scalable, SynthWorlds provides a controlled environment for evaluating LMs in ways that were previously challenging, enabling precise and testable comparisons of reasoning and memorization.

==> sections/prompts/direct-prompt.tex <==
% \subsection{Prompts}

\vspace{5pt}
\begin{prompt}[\textbf{Direct Prompting Baseline}]

\begin{systemmessage}
You are an expert-level data scientist. Your job is to answer a data analysis question in rigorous manner given a data table.
In your analysis: \\
\vspace*{0.5em}
{\small \textbullet} Carefully address \\
\begin{enumerate}[label=\arabic*), itemsep=0.0em, leftmargin=2.5em]
    \item Missing data: empty or null entries simulating incomplete information.
    \item Bad values: clearly erroneous or placeholder entries (e.g., \texttt{-1}, \texttt{9999}, \texttt{TEST}, \texttt{\#REF!}, etc.).
    \item Outliers: implausible extreme values that distort analysis (e.g., 220 breathing rate per minute).
    \item Inconsistent formatting: variations in representing the same value (e.g., \texttt{22 lbs}, \texttt{22 pounds}, \texttt{weight = 22}).
    \item Inconsistent logic: cross-field contradictions violating common-sense logic (e.g., end time before start time).
\end{enumerate}

    % \quad 1) missing data: empty or null entries simulating incomplete information \\
    % \quad 2) bad values: clearly erroneous or placeholder entries (e.g., `-1`, `9999`, `TEST`, `#REF!` etc.) \\
    % \quad 3) outliers: implausible extreme values that distort analysis (e.g., 220 breathing rate per minute) \\
    % \quad 4) inconsistent formatting: variations in representing the same value (e.g., `22 lbs`, `22 pounds`, `weight = 22`) \\
    % \quad 5) inconsistent logic: cross-field contradictions violating common-sense logic (e.g., end time before start time) \\
  {\small \textbullet} Attempt to safely recover or correct flawed data when reasonable based on the existing data. If data is irrecoverable or suspect, discard the row. \\
  {\small \textbullet} Do NOT write or execute any code. Focus purely on logical reasoning and analytical judgment. \\
  \vspace*{0.5em}
  You must conclude with your most reasonable answer. \\
  
  When you provide the final answer, please use the prefix "The answer is:" 
  without any modification, and provide the answer directly, with no formatting, no bolding, and \
  no markup. For instance: "The answer is: 42" or "The answer is: yes". If the question asks \
  for a list of values, then the answer should be a comma-separated list of values, \
  without any formatting, no bolding, and no markup. For instance: "The answer is: 42, 43, 44" or "The answer is: yes, no".
\end{systemmessage}

% \begin{fewshotexamples}
\begin{usermessage}
Data: \\
\begin{describedexample}{}{Example Table}
\begin{jsonblock}
race_year_id,race,time,time_in_seconds,runner
68140,Millstone 100,26H 35M 25S,95725.0,VERHEUL Jasper
68140,Millstone 100,27H 0M 29S,97229.0,MOULDING JON
68140,Millstone 100,28H 49M 7S,103747.0,RICHARDSON Phill
68140,Millstone 100,30H 53M 37S,111217.0,DYSON Fiona
68140,Millstone 100,32H 46M 21S,117981.0,FRONTERAS Karen
68140,Millstone 100,32H 46M 40S,118000.0,THOMAS Leigh
68140,Millstone 100,33H 30M 1S,120601.0,SHORT Deborah
68140,Millstone 100,33H 33M 23S,120803.0,CROSSLEY Catharine
68140,Millstone 100,34H 54M 16S,125656.0,BUTCHER Kent
68140,Millstone 100,34H 59M 39S,125979.0,Hendry Bill
68140,Millstone 100,34H 59M 44S,125984.0,Barnard Andrew
68140,Millstone 100,35H 19M 52S,127192.0,PAGE Mark
68140,Millstone 100,35H 34M 33S,128073.0,O'DONOGHUE Katie
71873,ElbrusWorldRace,29H 36M 14S,106574.0,ROSTOVTSEV Artem
71873,ElbrusWorldRace,33H 6M 45S,119205.0,Yakimov Semyon
71873,ElbrusWorldRace,36H 18M 2S,130682.0,Bolomozhnov Maksim
71873,ElbrusWorldRace,38H 4M 32S,137072.0,KUPRYUKHIN Denis
71873,ElbrusWorldRace,38H 4M 32S,137072.0,MITUSOV Viktor
71873,ElbrusWorldRace,40H 2M 34S,144154.0,OGURTSOV Aleksandr
...
\end{jsonblock}
\end{describedexample}
% 71873,ElbrusWorldRace,40H 44M 39S,146679.0,KUTS Aleksander
% 71873,ElbrusWorldRace,40H 54M 46S,147286.0,IVSHIN Mikhail
% 71873,ElbrusWorldRace,41H 7M 25S,148045.0,Frolov Valentin
% 71873,ElbrusWorldRace,41H 7M 26S,148046.0,Petrov Aleksandr
% 71873,ElbrusWorldRace,42H 5M 50S,151550.0,TIHONOV Aleksej
% =
Based on the given table, answer the following question: \\
\begin{describedexample}{}{Example Question}
\vspace{0.5em}
{\small In this dataset of ultra trail running race results, what is the average finishing time in minutes across all rows in the dataset?
Return your answer rounded to the nearest minute as an integer using bankers rounding (round half to even). Examples: round(2.5) $\rightarrow$ 2, round(3.5) $\rightarrow$ 4, round(4.3) $\rightarrow$ 4, round(4.7) $\rightarrow$ 5.}
\end{describedexample}
\end{usermessage}

% \begin{assistantmessage}
% \vspace{-1em}
% \begin{describedexample}{}{Example Output o4-mini (only completion tokens)}
% \vspace{0.5em}
% {\small The answer is: 2033}
% \end{describedexample}
% \end{assistantmessage}
\end{prompt}


\vspace{40pt}
\begin{prompt}[\textbf{Code Agent Baseline}]
\begin{systemmessage}
SETTING: \\
\vspace*{0.3em}
You are an expert-level data scientist. Your job is to answer a data analysis question in rigorous manner given a data table.
In your analysis: \\
\vspace*{0.5em}
{\small \textbullet} Carefully address \\
\begin{enumerate}[label=\arabic*), itemsep=0.0em, leftmargin=2.5em]
    \item Missing data: empty or null entries simulating incomplete information.
    \item Bad values: clearly erroneous or placeholder entries (e.g., \texttt{-1}, \texttt{9999}, \texttt{TEST}, \texttt{\#REF!}, etc.).
    \item Outliers: implausible extreme values that distort analysis (e.g., 220 breathing rate per minute).
    \item Inconsistent formatting: variations in representing the same value (e.g., \texttt{22 lbs}, \texttt{22 pounds}, \texttt{weight = 22}).
    \item Inconsistent logic: cross-field contradictions violating common-sense logic (e.g., end time before start time).
\end{enumerate}

    % \quad 1) missing data: empty or null entries simulating incomplete information \\
    % \quad 2) bad values: clearly erroneous or placeholder entries (e.g., `-1`, `9999`, `TEST`, `#REF!` etc.) \\
    % \quad 3) outliers: implausible extreme values that distort analysis (e.g., 220 breathing rate per minute) \\
    % \quad 4) inconsistent formatting: variations in representing the same value (e.g., `22 lbs`, `22 pounds`, `weight = 22`) \\
    % \quad 5) inconsistent logic: cross-field contradictions violating common-sense logic (e.g., end time before start time) \\
  {\small \textbullet} Attempt to safely recover or correct flawed data when reasonable based on the existing data. If data is irrecoverable or suspect, discard the row. \\
  \vspace*{0.5em}
  You will be working within a Python shell and can use the following commands to answer the question. \\
 \vspace*{1.0em}
AVAILABLE COMMANDS:
{\scriptsize		
\begin{jsonblock}
python:
  docstring: Execute Python code within a persistent Python shell. The shell maintains
    state across executions, so variables and imports from previous runs remain available.
    When first using this command, the data table is provided as a global variable
    named `df`, and `pandas` has already been imported as `pd`.
  arguments:
  - name: code
    arg_type: str
    description: The Python code to execute.
    required: true
  demonstration: "```\ncommand: python\nkwargs:\n  code: <arg value>\n```"
done:
  docstring: Indicate that we arrived at the final answer and provide the answer.
    Use this command only when you have arrived at the final answer.
  arguments:
  - name: answer
    arg_type: str
    description: The final answer to the question. Do not apply any formatting, bolding,
      or markup. If the question asks for a list of values, then the answer should
      be a comma-separated list of values (e.g., '42, 43, 44')
    required: true
  demonstration: "```\ncommand: done\nkwargs:\n  answer: <arg value>\n```"
\end{jsonblock}
}
\vspace*{0.5em}
RESPONSE\_FORMAT: \\
\vspace*{0.3em}
Each response must include:
\begin{enumerate}[label=\arabic*), itemsep=0.0em, leftmargin=2.5em]
\item A DISCUSSION field — where you will methodically break down the reasoning process, illustrating how you arrive at conclusions and decide what to do next.
\item A command field — properly formatted YAML within triple backticks and following the structure from COMMANDS.
\end{enumerate}

Important rules: \\
\begin{itemize}[label=-, itemsep=0.0em, leftmargin=1.5em]
  \item Always include exactly one DISCUSSION and one command block.
  \item Ensure the command block is properly formatted YAML with proper indents and newlines (see the example below).
\end{itemize}
For example, given a question asking for the average income. You might respond: \\
\vspace*{0.5em}
DISCUSSION \\
\vspace*{0.3em}
Let's think step by step. We need to first find the average income of the population. We can do this by summing up the income column and dividing by the number of rows.
{\scriptsize
\begin{jsonblock}
```yaml
  command: "python"
  kwargs:
    code: |-
      income_avg = df['income'].sum() / len(df)
      income_avg
```
\end{jsonblock}
}
\end{systemmessage}

% \begin{fewshotexamples}
\begin{usermessage}
Begin! \\
\vspace{1.0em}
Data table (stored in a pandas dataframe named `df`): \\
\begin{describedexample}{}{Example Table}
\begin{jsonblock}
RideID,payment_type,lpep_pickup_datetime,lpep_dropoff_datetime,passenger_count,trip_distance,tolls_amount,mta_tax,start_day_of_week,store_and_fwd_flag
239022,2.0,04/10/2021 11:11:55 AM,04/10/2021 11:18:14 AM,1.0,1.1,0.0,0.5,Saturday,N
926728,1.0,11/27/2021 01:13:13 PM,11/27/2021 01:21:26 PM,1.0,1.77,0.0,0.5,Saturday,N
761139,1.0,10/06/2021 12:13:08 AM,10/06/2021 12:36:37 AM,1.0,4.59,0.0,0.5,Wednesday,N
701071,2.0,09/24/2021 05:03:11 PM,09/24/2021 05:33:50 PM,1.0,3.67,0.0,0.5,Friday,N
700330,1.0,09/24/2021 12:32:02 PM,09/24/2021 01:01:23 PM,1.0,6.43,0.0,0.5,Friday,N
676804,1.0,09/13/2021 03:12:04 PM,09/13/2021 03:25:17 PM,17.0,2.23,0.0,0.0,Monday,N
245344,1.0,04/14/2021 06:00:15 PM,04/14/2021 06:07:14 PM,1.0,1.45,0.0,0.5,Wednesday,N
763937,1.0,10/07/2021 08:52:44 AM,10/07/2021 09:18:10 AM,1.0,2.38,0.0,0.5,Thursday,N
906875,1.0,11/19/2021 08:13:35 AM,11/19/2021 08:25:17 AM,32.0,1.3,0.0,0.5,Friday,N
452863,1.0,06/30/2021 07:48:41 AM,06/30/2021 07:58:07 AM,1.0,1.4,0.0,0.5,Wednesday,N
799361,2.0,10/21/2021 08:11:35 PM,10/21/2021 08:25:35 PM,1.0,2.7,0.0,0.5,Thursday,N
778926,1.0,10/13/2021 04:48:46 PM,10/13/2021 05:04:11 PM,1.0,1.94,0.0,0.5,Wednesday,N
701648,2.0,09/24/2021 09:41:56 PM,09/24/2021 09:46:04 PM,1.0,0.68,0.0,0.5,Friday,N
658773,1.0,09/03/2021 06:04:46 PM,09/03/2021 06:31:10 PM,1.0,6.81,6.55,0.5,Friday,N
1011851,1.0,12/16/2021 08:04:25 PM,12/16/2021 08:17:31 PM,1.0,2.61,6.55,0.5,Thursday,N
798988,1.0,10/21/2021 06:38:26 PM,10/21/2021 06:49:36 PM,2.0,1.9,0.0,0.5,Thursday,N
1041391,1.0,12/30/2021 09:26:36 PM,12/30/2021 09:46:14 PM,32.0,8.38,0.0,0.5,Thursday,N
150322,2.0,03/07/2021 01:46:05 PM,03/07/2021 01:58:56 PM,1.0,2.78,0.0,0.5,Sunday,N
1042470,2.0,12/31/2021 02:16:09 PM,12/31/2021 02:23:56 PM,1.0,1.1,0.0,0.5,Friday,N
320608,1.0,05/06/2021 04:00:07 PM,05/06/2021 04:13:59 PM,2.0,1.8,0.0,0.5,Thursday,N
101586,1.0,02/21/2021 11:54:04 AM,02/21/2021 11:59:48 AM,17.0,0.89,0.0,0.5,Sunday,N
802662,2.0,10/23/2021 08:09:51 AM,10/23/2021 08:21:26 AM,1.0,5.13,0.0,0.5,Saturday,N
536010,2.0,07/30/2021 08:24:30 PM,07/30/2021 08:36:58 PM,5.0,1.48,0.0,0.5,Friday,N
1014944,2.0,12/17/2021 11:21:29 PM,12/17/2021 11:28:04 PM,1.0,1.1,0.0,0.5,Friday,N
683930,1.0,09/16/2021 10:55:54 PM,09/16/2021 11:21:57 PM,1.0,6.7,0.0,0.5,Thursday,N
776498,1.0,10/12/2021 05:46:33 PM,10/12/2021 06:01:26 PM,2.0,2.2,0.0,0.5,Tuesday,N
...
\end{jsonblock}
\end{describedexample}
All cells in the `df` are `object` data type, regardless of their appearance. \\

Question: \\
\begin{describedexample}{}{Example Question}
\vspace{0.5em}
{\small How many total passengers were there from the trips in the dataset?}
\end{describedexample}
\end{usermessage}
% \vspace{3em}
% \begin{assistantmessage}
% \vspace{-1em}
% \begin{describedexample}{}{Example Output Gemini 2.5 Flash}
% \vspace{0.5em}
% {\scriptsize	
% DISCUSSION \\
% The user wants to know the total number of passengers across all trips in the dataset. \\
% The `passenger\_count` column contains the number of passengers for each trip. \\
% I need to sum the values in the `passenger\_count` column. \\
% Before summing, I need to address potential data quality issues in the `passenger\_count` column: \\
% \begin{enumerate}[itemsep=0.0em, leftmargin=2.5em]
%   \item **Missing data:** Check for null or empty values.
%   \item **Bad values:** Look for non-numeric entries or placeholder values like -1.
%   \item **Outliers:** Identify implausibly high passenger counts (e.g., 17, 32). While these might be real (e.g., shared rides or data entry errors), they are significantly higher than typical taxi/rideshare passenger counts. Given the context of a standard taxi/rideshare, counts like 17 and 32 seem highly unlikely and are likely data errors. I will treat these as outliers and remove the corresponding rows. A reasonable upper limit for passenger count in a standard vehicle might be around 6-8. I will remove rows where `passenger\_count` is greater than 8.
%   \item **Inconsistent formatting:** The data is provided as `object` type, so I need to convert `passenger\_count` to a numeric type (float or integer) before summing.
%   \item **Inconsistent logic:** No obvious logical inconsistencies related to passenger count with other columns.
% \end{enumerate}
% Steps:
% \begin{enumerate}[itemsep=0.0em, leftmargin=2.5em]
%   \item Convert the `passenger\_count` column to a numeric type, coercing errors to NaN.
%   \item Handle missing values (NaNs) by dropping rows with missing `passenger\_count`.
%   \item Identify and remove rows where `passenger\_count` is greater than 8.
%   \item Sum the remaining values in the `passenger\_count` column.
%   \item Convert the sum to an integer as passenger counts are whole numbers.
%   \item Provide the final sum as the answer.
% \end{enumerate}

% \begin{jsonblock}
% ```yaml
% command: python
% kwargs:
%   code: |-
%     # Convert passenger_count to numeric, coercing errors
%     df['passenger_count'] = pd.to_numeric(df['passenger_count'], errors='coerce')

%     # Drop rows with missing passenger_count
%     df.dropna(subset=['passenger_count'], inplace=True)

%     # Remove rows with passenger_count > 8 (outliers)
%     df = df[df['passenger_count'] <= 8]

%     # Calculate the sum of passenger_count
%     total_passengers = df['passenger_count'].sum()

%     # Convert to integer
%     total_passengers = int(total_passengers)

%     print(total_passengers)
% ```
% \end{jsonblock}
% }
% \end{describedexample}
% \end{assistantmessage}
\end{prompt}

